GLM-4-Voice: Towards Intelligent and Human-Like End-to-End Spoken Chatbot

We introduce GLM-4-Voice, an intelligent and human-like end-to-end spoken chatbot. It supports both Chinese and English, engages in real-time voice conversations, and varies vocal nuances such as emotion, intonation, speech rate, and dialect according to user instructions. GLM-4-Voice uses an ultra-low bitrate (175bps), single-codebook speech tokenizer with 12.5Hz frame rate derived from an automatic speech recognition (ASR) model by incorporating a vector-quantized bottleneck into the encoder. To efficiently transfer knowledge from text to speech modalities, we synthesize speech-text interleaved data from existing text pre-training corpora using a text-to-token model. We continue pre-training from the pre-trained text language model GLM-4-9B with a combination of unsupervised speech data, interleaved speech-text data, and supervised speech-text data, scaling up to 1 trillion tokens, achieving state-of-the-art performance in both speech language modeling and spoken question answering. We then fine-tune the pre-trained model with high-quality conversational speech data, achieving superior performance compared to existing baselines in both conversational ability and speech quality. The open models can be accessed through https://github.com/THUDM/GLM-4-Voice and https://huggingface.co/THUDM/glm-4-voice-9b.

==> tables/speech_decoder.tex <==
\begin{table}[ht]
\centering
% \setlength{\tabcolsep}{0.5\tabcolsep}
\caption{\textbf{Speech Tokenizer Results}. We evaluate semantic retention (Expresso, LS) and reconstruction quality (VisQOL, MOSNet) for different speech tokenizers across various sample rates. \todo{Reformat this table or replace it with a figure}}
% \resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Tokenizer}} & \multirow{2}{*}{{\shortstack{\textbf{Sample}\\\textbf{Rate}}}} & \multirow{2}{*}{\textbf{Bitrate}} & \multirow{2}{*}{\textbf{Causal}} & \multicolumn{2}{c}{\textbf{Content}$\downarrow$} & \multicolumn{2}{c}{\textbf{Quality}$\uparrow$} \\
\cmidrule(lr){5-6} \cmidrule(lr){7-8}
 & &  &  & Expresso & LS & VisQOL & MOSNet \\
\midrule
Ground Truth & - & - & - & 15.83 & 4.62 & - & 3.27 \\
RVQGAN & 75Hz & 1.50K & \xmark & - & - & 1.74 & 2.74 \\
SemantiCodec & 50Hz & 1.30K & \xmark & - & - & 2.43 & 3.12 \\
SpeechTokenizer & 50Hz & 1.50K & \xmark & - & - & 1.53 & 2.67 \\
SpeechTokenizer & 50Hz & 4.00K & \xmark & - & - & 3.07 & 3.10 \\
Spirit-Base & 25Hz & 225.0 & \xmark & 22.90  & 11.66  & - & - \\
Spirit-Expressive & 38.5Hz & 307.0 & \xmark & 22.35  & 10.60  & - & - \\
Moshi (Mimi) & 12.5Hz & 1.10K & \cmark & 21.00   & 8.36   & 2.82 & 2.89 \\
\midrule
\multirow{4}{*}{Ours} & 50Hz & 180.6 & \cmark & 17.77 & 6.24  & 2.67 &3.38 \\
 & 25Hz & 90.3 & \cmark & 17.78  &6.80   & 2.60 & 3.33 \\
 & 12.5Hz & 52.7 & \cmark &19.88    &8.43    & 2.52 & 3.39 \\
 & 6.25Hz & 30.1 & \cmark &24.21    & 14.41  & 2.34 & 3.24 \\
\bottomrule
\end{tabular}
% }
\label{tab:speech_decoder}
\end{table}
